PhysGNN: A Physics-Driven Graph Neural Network Based Model for Predicting Soft Tissue Deformation in Image-Guided Neurosurgery

Correctly capturing intraoperative brain shift in image-guided neurosurgical procedures is a critical task for aligning preoperative data with intraoperative geometry for ensuring accurate surgical navigation. While the finite element method (FEM) is a proven technique to effectively approximate soft tissue deformation through biomechanical formulations, their degree of success boils down to a trade-off between accuracy and speed. To circumvent this problem, the most recent works in this domain have proposed leveraging data-driven models obtained by training various machine learning algorithms -- e.g., random forests, artificial neural networks (ANNs) -- with the results of finite element analysis (FEA) to speed up tissue deformation approximations by prediction. These methods, however, do not account for the structure of the finite element (FE) mesh during training that provides information on node connectivities as well as the distance between them, which can aid with approximating tissue deformation based on the proximity of force load points with the rest of the mesh nodes. Therefore, this work proposes a novel framework, PhysGNN, a data-driven model that approximates the solution of the FEM by leveraging graph neural networks (GNNs), which are capable of accounting for the mesh structural information and inductive learning over unstructured grids and complex topological structures. Empirically, we demonstrate that the proposed architecture, PhysGNN, promises accurate and fast soft tissue deformation approximations, and is competitive with the state-of-the-art (SOTA) algorithms while promising enhanced computational feasibility, therefore suitable for neurosurgical settings.

==> paper/present_work_old.tex <==
\noindent \textbf{Present Work.} In this work, we propose a novel data-driven framework, named PhysGNN\footnote{The data and implementation will be made available at https://github.com/TBA}, which is based on two types of Graph Neural Networks (GNNs) \cite{scarselli2008graph}, namely GraphSAGE- \cite{hamilton2017inductive} and GraphConv \cite{morris2019weisfeiler}, that is trained with the results of Finite Element Analysis (FEA), and thus is based on the physical characteristics of soft tissue. The motivation behind using GNNs for capturing tissue deformation upon prescibed loads is their ability to define deep neural networks on graph data. Specifically, GNNs are a class of node embedding techniques\footnote{Node embedding techniques are a set of approaches that encode graph data---e.g. nodes, edges, features---into a lower dimensional vector space \cite{hamilton2017representation}.} that enable generalization of convolution on graph data through the notion of \textit{neural message passing} \cite{gilmer2017neural}, by which the information of nodes within a neighbourhood of an arbitrary size are transformed and aggregated producing a new value \cite{hamilton2020graph}. The message passing framework enables inductive learning over graphs through \textit{parameter sharing}, a property that ensures learning a constant number of parameters independent of the mesh size. Therefore, contrary to the previous methods, not only is PhysGNN capable of incorporating mesh structural information---i.e. proximity of mesh nodes with each other and the Euclidean distance of neighbouring nodes from one another---which can aid with effective prediction of tissue deformation, but also enhances computational feasibility when learning from high quality meshes that consist of many nodes. To the best of our knowledge, we are the first ones to leverage GNNs for approximating soft tissue deformation under prescribed forces. 

We evaluate the performance of PhysGNN on two datasets, which are distinguished by the number of force load points and the total force applied, where our baseline is the results of FEA. Through our empirical results, we demonstrate that PhysGNN is capable of successfully predicting tissue deformation upon prescibed forces under 0.005 and 1.9 seconds using a GPU and CPU, respectively. In fact, the absolute displacement error of PhysGNN for 97\% of the nodes is found be be under 1 mm---which is the precision in neurosurgery \cite{miller2010biomechanics}. 
